Metric on Nonlinear Dynamical Systems with Perron-Frobenius Operators

The development of a metric for structural data is a long-term problem in pattern recognition and machine learning. In this paper, we develop a general metric for comparing nonlinear dynamical systems that is defined with Perron-Frobenius operators in reproducing kernel Hilbert spaces. Our metric includes the existing fundamental metrics for dynamical systems, which are basically defined with principal angles between some appropriately-chosen subspaces, as its special cases. We also describe the estimation of our metric from finite data. We empirically illustrate our metric with an example of rotation dynamics in a unit disk in a complex plane, and evaluate the performance with real-world time-series data.

==> background.tex <==
\section{Background}
\label{sec:background}

%-----
\subsection{Reviews on Existing Metrics for Dynamical Systems}
\label{ssec:metric_lds}

Here, we review two major metrics for dynamical systems. As mentioned in the introduction, Martin ... De Cock nd De Moor ...

%Wolf and Shashua demonstrated how subspace angles can be efficiently computed by using kernel methods~\cite{WS03}. In related work, Shashua and Hazan show how tensor products can be used to construct a general family of kernels on sets \cite{SH05}. Hamm~and~Lee ... \cite{HL08}.


%-----
\input{koopman}

==> estimation.tex <==
\section{Estimation from Finite Data}
\label{sec:est}

(===== Describe here the case with reproducing kernels and data sequences =====)

(==draft by KF==)

We consider $\{x_{j}(0)^{i}, x_j^i(1), x_j^i(2), \dots\}\subset X_i$ ($j=1,\dots, N$) where each $X_i$ is $N$ finite-length sequences. 
Moreover, we assume
\[f_i\left(x_{j}^{i}(t)\right)=x_{j}^i(t+1).\]
Now, we define $\bfb{g}_i: H\rightarrow \cpxnum^N$:
\[\bfb{g}_i(v):=\left( \left\langle v,\,\phi\left(x_{1}^i(0)\right)\right\rangle, \dots,\left\langle v,\,\phi\left(x_{N}^i(0)\right)\right\rangle\right).\]
Then, for each $m=1,\dots, N$, we have
\begin{align}\label{eq:estimation}
&I_T^{(m)}((K_i, \bfb{g}_i), (K_j, \bfb{g}_j))\\
&=\sum_{t_1=0}^T\dots\sum_{t_m=0}^T\sum_{0<s_1<\dots<s_m\le N}
\det\left(
\begin{array}{ccc}
k\left(x_{s_1}^i(t_1),\,x_{s_1}^j(t_1)\right)&\cdots&k\left(x_{s_1}^i(t_1),\,x_{s_m}^j(t_m)\right)\\
\vdots&\ddots&\vdots\\
k\left(x_{s_m}^i(t_m),\,x_{s_1}^j(t_1)\right)&\cdots&k\left(x_{s_m}^i(t_m),\,x_{s_m}^j(t_m)\right)
\end{array}
\right)\nonumber.
\end{align}
Therefore, we can compute $A_m$ by calculating the limit on $T$ of this quotient described in the definition 3.1 (The derivation is shown in Appendix A). 

